On Improving the Composition Privacy Loss in Differential Privacy for Fixed Estimation Error

This paper considers the private release of statistics of disjoint subsets of a dataset, in the setting of data heterogeneity, where users could contribute more than one sample, with different users contributing potentially different numbers of samples. In particular, we focus on the $\epsilon$-differentially private release of sample means and variances of sample values in disjoint subsets of a dataset, under the assumption that the numbers of contributions of each user in each subset is publicly known. Our main contribution is an iterative algorithm, based on suppressing user contributions, which seeks to reduce the overall privacy loss degradation under a canonical Laplace mechanism, while not increasing the worst estimation error among the subsets. Important components of this analysis are our exact, analytical characterizations of the sensitivities and the worst-case bias errors of estimators of the sample mean and variance, which are obtained by clipping or suppressing user contributions. We test the performance of our algorithm on real-world and synthetic datasets and demonstrate clear improvements in the privacy loss degradation, for fixed worst-case estimation error.

==> alg.tex <==
\label{sec:alg}
%Prajjwal: In this section we first describe three components used to build our algorithm (Algorithm X) and then present our final algorithm.

In this section, we present 4 algorithms: \textsc{Baseline}, \textsc{Array-Averaging}, \textsc{Levy}, and \textsc{Quantile}, for private mean estimation with user-level privacy. These algorithms are designed keeping in mind their intended application, which is to analyze speed values of buses in large cities. Before we do so, we describe a useful approach that modifies the function $f$ to be estimated (see \eqref{eq:f}), in order to reduce the dependence of the standard deviation of the noise added on the number of samples per user (see the discussion at the end of the previous section): we clip the number of samples contributed by any user $\ell\in [L]$ to $\min\{m_\ell,m_\text{UB}\}$, where $m_\star\leq m_\text{UB}\leq m^\star$ is some fixed constant that depends on $\{m_\ell\}_{\ell\geq 1}$. We describe next two such so-called ``grouping" strategies, inspired by the work in \cite{tyagi}: \textsc{WrapAround} and \textsc{BestFit}.
\subsection{Strategies for Grouping Samples}
\label{sec:grouping}
Let $m_{\text{UB}}$ be given. The procedure underlying grouping strategies is as follows: for ease of exposition, we first sort the users in non-increasing order of the number of samples contributed, i.e., we reindex the users so that $m_1\geq m_2\geq\ldots\geq m_L$. We then initialize $L$ empty arrays $A_1,\ldots,A_L$, each of length $m_{\text{UB}}$. We assume that the locations of the arrays are indexed from 1 to $m_\text{UB}$, and for a given array $A$, we use the notation $w(A)$ to denote the number of filled locations. We initialilze $w(A_i) = 0$, for all $1\leq i\leq L$. Now, we process each user in turn, beginning with user 1 and populate his/her samples in the arrays, with a maximum of $m_\text{UB}$ samples from any user being populated in the arrays. The exact strategy for populating arrays followed in the \textsc{WrapAround} and \textsc{BestFit} procedures is explained below.
\subsubsection{\textsc{WrapAround}}
Let $\ell^*$ denote the smallest value of $\ell\in [L]$ such that $m_\ell < m_\text{UB}$. For every $\ell<\ell^*$, we populate the array $A_\ell$ with the speed samples $\left(S_j^{(\ell)}: 1\leq j\leq m_\text{UB}\right)$, in a contiguous manner. Next, we pick the samples $\left(S_j^{(\ell^\star)}: 1\leq j\leq m_{\ell^\star}\right)$ from user $\ell^\star$ and add these to array $A_{\ell^\star}$ contiguously. By the definition of $\ell^\star$, there exist some empty slots in array $A_{\ell^\star}$. These are filled completely by the next user's samples $\left(S_j^{(\ell^\star+1)}: 1\leq j\leq m_{\ell^\star+1}\right)$, if $m_{\ell^\star+1}\leq m_\text{UB}-m_{\ell^\star}$ contiguously; else, these slots are filled by the samples $\left(S_j^{(\ell^\star+1)}: 1\leq j\leq m_\text{UB}-m_{\ell^\star}\right)$, and the remaining samples from user $\ell^\star+1$ are filled in the first $m_{\ell^\star+1}+m_{\ell^\star} - m_{\text{UB}}$ positions of array $A_{\ell^\star+1}$. The procedure then continues, filling each array in turn, until all the user's samples have been populated in the arrays. Let $K$ denote the index of the last filled-up array, with the arrays $A_{K+1},\ldots,A_L$ being deleted. Note that
\begin{equation}
	\label{eq:K}
K = \left \lfloor \frac{\sum_{\ell=1}^{L}\min \left \{m_{\ell}, m_\text{UB} \right \}}{m_\text{UB}} \right \rfloor.
\end{equation}
Observe that in this strategy, it can happen that the samples from a given user $\ell\in [L]$ are split between two arrays $A_i$ and $A_{i+1}$, for some $1\leq i\leq K-1$; we then say that this user $\ell$ ``influences'' two arrays. The \textsc{WrapAround} strategy is shown as Algorithm \ref{alg:wrap}.
%We first create $k$ arrays of user samples following the approach in Algorithm 7 presented in [GRST22]. The main idea is to group user samples into $k$ arrays of size $l$ such that each array contains enough diversity to exploit any concentration of the underlying unknown distribution. The requirement is that the mean $Z_{i}$ of array $S_{i}, i \in [k]$ is a coarse estimate of the true empirical mean $\mu$. We set $l$ to be the \textit{median} of the number of samples contributed by users. Thus for $m_{i} = \left | x_{i}\right |, i \in [n]$ we have $l = Median({m_{1}, m_{2}, ..., m_{n}})$. We use the median of values as it would ensure that at least half the arrays are completely filled by samples from a user.

% Explain why median, what is the benefit/motivation
% Mention how k is calculated
% Clarify what is good enough coarse estimate, how to achieve that in non iid
% Mention any requirements on number of users and number of samples for the algorithm to work

\subsubsection{\textsc{BestFit}}

This algorithm that we use is a version of a popular online algorithm for the bin-packing problem, which is a known strongly NP-complete problem (see \cite{np}). Similar to the description of \textsc{WrapAround}, let $\ell^*$ denote the smallest value of $\ell\in [L]$ such that $m_\ell < m_\text{UB}$. For every $\ell<\ell^*$, we populate the array $A_\ell$ with the speed samples $\left(S_j^{(\ell)}: 1\leq j\leq m_\text{UB}\right)$, in a contiguous manner. For each user $\ell\geq \ell^\star$, we find the least-indexed array $A$ among $A_{\ell^\star},\ldots,A_L$ that can accommodate $m_\ell$ samples and is filled the most. The $m_\ell$ samples from the user $\ell$ are then placed in array $A$ (in a continguous manner), and the process is iterated over the other users. Note that the number of non-empty arrays that are returned by the \textsc{BestFit} algorithm $\overline{K}$, is at least $K$ (see \eqref{eq:K}). Furthermore, observe that the samples from any given user $\ell\in [L]$ are present in exactly one array, unlike the case in the \textsc{WrapAround} strategy. Hence, any user influences at most one array, in this case.

The \textsc{BestFit} strategy is shown as Algorithm \ref{alg:bestfit}.

%Prajjwal: We note that the sample grouping discussed in [GRST22] allows for samples by one user be stored in more than one array. In order to create a set of completely filled arrays, we set $k$ to be $\left \lfloor \frac{\sum_{i=1}^{n}min \left \{m_{i}, l \right \}}{l} \right \rfloor$. Note that in this approach, one user's samples can affect two arrays and hence, their corresponding means $Z_{i}$. This leads to the sensitivity of the subsequent exponential mechanism used for private interval estimate, discussed in \textit{Section B}, to be increased by a factor 2. This can have a significant impact on the utility of the resulting algorithm as demonstrated empirically in the results section of this paper.To mitigate this effect, we propose the use of best fit algorithm in \textsc{BestFitGrouping} discussed as a solution to the bin-packing problem. In \textsc{BestFitGrouping} algorithm, the arrays are dynamically created as per predefined conditions. Note that it is not necessary the the arrays returned by this algorithms will be completely filled. However, it ensures that at most one array can have less than $l/2$ samples. 

% Change sensitivity to a more specific term as it is vague/wrong. Tell in terms of Delta
% Write one line about the best-fit algorithm
% Explain that in best-fit some arrays may not be completely filled. Atmost one array could be filled less than l/2



\begin{algorithm}
	\caption{The wrap-around strategy}
	\begin{algorithmic}[1]
		\Procedure {\textsc{WrapAround}}{$\mathcal{D}, m_\text{UB}$}
		
		\State Set $K \gets \left \lfloor \frac{\sum_{\ell=1}^{L}\min \left \{m_{\ell}, m_\text{UB} \right \}}{m_\text{UB}} \right \rfloor$.
		\State Initialize $t\gets 1$
		\For {$\ell= 1:L$}
		\State Set $r \gets \min\left \{m_{\ell}, m_\text{UB} \right \}$, $w \gets w(A_t)$.
		\If {$m_\text{UB}-w\geq r$}
		\State Fill $A_t(w+1:w+r) = \left(S_1^{(\ell)},\ldots, S_r^{(\ell)}\right)$
		\Else
		\State Fill $A_t(w+1:m_\text{UB}) = \left(S_1^{(\ell)},\ldots, S_{m_\text{UB}-w}^{(\ell)}\right)$.
		\State Update $t\gets t+1$, set $r' = r+w-m_\text{UB}$.
		\State Fill $A_t(1:r') = \left(S_{m_\text{UB}-w+1}^{(\ell)},\ldots, S_r^{(\ell)}\right)$.
		\EndIf
		\EndFor
		\State \Return $A_{1}, \ldots, A_{K}$
		\EndProcedure
	\end{algorithmic}
	\label{alg:wrap}
\end{algorithm}


\begin{algorithm}
	\caption{The best-fit strategy}
	\begin{algorithmic}[1]
		\Procedure{BestFit}{$\mathcal{D}, m_\text{UB}$}
		\For {$\ell \leftarrow 1:L$}
		\State Set $r \gets \min\left \{m_{\ell}, m_\text{UB}\right\}$
		\State Set $\mathcal{A} = \{A_i: m_\text{UB}-w(A_i)\geq r\}$.
		\State Set $A = A_j\in \mathcal{A}$ such that $j$ is the least index such that $w(A_j) = \max_{A'\in \mathcal{A}} w(A')$.
		\State Fill $A(w(A)+1:r+w(A)) = (S_1^{(\ell)},\ldots, S_r^{(\ell)})$.
		\EndFor
		\State \Return non-empty arrays $A_{1}, \ldots,A_{\overline{K}}$
		\EndProcedure
	\end{algorithmic}
\label{alg:bestfit}
\end{algorithm}

With these grouping strategies in place, we shall now describe our main algorithms.

\subsection{\textsc{Baseline}}
\label{sec:baseline}
The \textsc{Baseline} algorithm simply adds the required amount of Laplace noise to guarantee $\varepsilon$-DP, to the function $f$ to be computed, i.e.,
\[
M_\text{Baseline}(\mathcal{D}) = f(\mathcal{D})+\text{Lap}(\Delta_f/\varepsilon),
\]
where $\Delta_f = \frac{Um^\star}{\sum_\ell m_\ell}$ is the sensitivity of the function $f$. As mentioned earlier, this algorithm suffers from the drawback that a large amount of noise needs to be added for privacy when either $U$ or $m^\star$ is large, thereby impeding estimation.

\subsection{\textsc{Array-Averaging}}

In this algorithm, we attempt to reduce the amount of noise added when $m^\star$ is large, by clipping the number of samples contributed by any given user to some $m_\star\leq m_\text{UB}\leq m^\star$. We use one of the two grouping strategies discussed previously: \textsc{WrapAround} or \textsc{BestFit} for clipping. In particular, given the database $\mathcal{D}$, we set

\[
f_\text{arr, wrap}(\mathcal{D}):=\frac{1}{K}\cdot \sum_{i=1}^K \overline{A_i},
\]
where $A_i$ are the arrays obtained using the \textsc{WrapAround} strategy, with $\overline{A_i}:= \frac{1}{w(A_i)} \sum_{j=1}^{w(A_i)} A_i(j)$ being the mean of the samples contributed by array $i\in [K]$. We also set
\[
 f_\text{arr, best}(\mathcal{D}):=\frac{1}{\overline{K}}\cdot \sum_{i=1}^{\overline{K}} \overline{A_i},
\]
 where $A_i$ are the arrays obtained using the \textsc{BestFit} strategy, with $\overline{A_i}:= \frac{1}{w(A_i)} \sum_{j=1}^{w(A_i)} A_i(j)$ being the mean of the samples contributed by array $i\in [\overline{K}]$.
 
 From the discussion in Section \ref{sec:grouping}, we have that since using the \textsc{WrapAround} strategy can result in one user influencing two arrays, the sensitivity is given by
 \begin{equation*}
 \Delta_{f_\text{arr, wrap}} = \frac{2U}{K}.
 \label{eq:delfwrap}
 \end{equation*}
However, since using the \textsc{BestFit} strategy, any user influences at most array, the sensitivity is 
 \begin{equation}
	\Delta_{f_\text{arr, best}} = \frac{U}{\overline{K}}.
	\label{eq:delfbest}
\end{equation}

The \textsc{Array-Averaging} algorithm with \textsc{WrapAround} grouping computes
\[
M_\text{ArrayAvg, wrap}(\mathcal{D}) = f_\text{arr, wrap}(\mathcal{D})+\text{Lap}(\Delta_{f_\text{arr, wrap}}/\varepsilon),
\]
and the \textsc{Array-Averaging} algorithm with \textsc{BestFit} grouping computes
\[
M_\text{ArrayAvg, best}(\mathcal{D}) = f_\text{arr, best}(\mathcal{D})+\text{Lap}(\Delta_{f_\text{arr, best}}/\varepsilon).
\]
Clearly, both these algorithms are $\varepsilon$-DP, from Theorem \ref{thm:dp}.

Observe that since $\overline{K}\geq K$, we have that $\Delta_{f_\text{arr, best}}\leq \frac{U}{K}< \Delta_{f_\text{arr, wrap}}$. This suggests that using the \textsc{BestFit} grouping strategy yields lower estimation error, since the corresponding standard deviation of the noise added is lower by a multiplicative factor of $2$ compared to the \textsc{WrapAround} strategy. In what follows, we therefore focus our attention on the \textsc{BestFit} strategy.

We now define
\[
\tilde{\Delta}_{f_\text{arr}}:= \frac{U \, m_\text{UB}}{\sum_{\ell=1}^L \min\{m_\ell, m_\text{UB}\}}
\]
as a proxy for the upper bound $U/K$ on $\Delta_{f_\text{arr, best}}$. If $\tilde{\Delta}_{f_\text{arr}}$ is small, then so are $U/K$ and $\Delta_{f_\text{arr, best}}$.
%\[
%f_\text{arr}(\mathcal{D}):= \frac{1}{\sum_{\ell=1}^L \min\{m_\ell, m_\text{UB}\}}\cdot \sum_{\ell=1}^L \min\{m_\ell, m_\text{UB}\}\cdot  \overline{S}^{(\ell)},
%\]
%where $\overline{S}^{(\ell)}:= \frac{1}{m_\ell} \sum_{j=1}^{m_\ell} S_j^{(\ell)}$ is the mean of the samples contributed by user $\ell\in [L]$. Note that since $\overline{S}^{(\ell)}\in (0,U]$, we have that the sensitivity
%\begin{equation}
%\Delta_{f_\text{arr}} = \frac{Um_\text{UB}}{\sum_{\ell=1}^L \min\{m_\ell, m_\text{UB}\}}.
%\label{eq:delfarr}
%\end{equation}


The following lemma, that compares the \textsc{Baseline} and \textsc{Array-Averaging} algorithms, then holds:

\begin{lemma}
	For any $m_\text{UB}\leq m^\star$, we have that $\Delta_f \geq \tilde{\Delta}_{f_\text{arr}}$.
\end{lemma}
\begin{proof}
	We need only prove that $\frac{m^\star}{\sum_\ell m_\ell}\geq \frac{m_\text{UB}}{\sum_{\ell=1}^L \min\{m_\ell, m_\text{UB}\}}$, or equivalently, that $\frac{m^\star}{m_\text{UB}}\geq \frac{\sum_\ell m_\ell}{\sum_{\ell=1}^L \min\{m_\ell, m_\text{UB}\}}$. To see this, let $B:= \{\ell\in [L]: m_\ell< m_\text{UB}\}$ and $B^c:= [L]\setminus B$. Then,
	\begin{align*}
		\frac{\sum_\ell m_\ell}{\sum_{\ell=1}^L \min\{m_\ell, m_\text{UB}\}}&= \frac{\sum_{\ell\in B} m_\ell + \sum_{\ell\in B^c} m_\ell }{\sum_{\ell\in B} m_\ell + \sum_{\ell\in B^c} m_\text{UB}}\\
		&\leq \frac{\sum_{\ell\in B^c} m_\ell }{|B^c|\cdot m_\text{UB}}\\
		&\leq \frac{m^\star}{m_\text{UB}},
	\end{align*}
where the first inequality holds since $\sum_{\ell\in B^c} m_\ell \ge \sum_{\ell\in B^c} m_\text{UB}$, and the second inequality holds since $m_\ell\leq m^\star$, for all $\ell\in [L]$.
\end{proof}
%From the above lemma, it is clear that the estimation error due to privacy using \textsc{Array-Averaging} is at most that using \textsc{Baseline}.
%
Next, we shall embark on choosing a ``good'' $m_\text{UB}$, which provides a large ``gain" $\frac{\Delta_f}{\tilde{\Delta}_{f_\text{arr}}}$; this therefore guarantees that $\Delta_{f_\text{arr, best}}$ is small.

To this end, call $\alpha:= \frac{m^\star}{m_\text{UB}}$; in our setting, we have $\alpha\geq 1$. For fixed $\{m_\ell\}_\ell\geq 1$, observe that
\begin{align*}
	\frac{\Delta_f}{\tilde{\Delta}_{f_\text{arr}}}&= \frac{\alpha}{\sum_\ell m_\ell}\cdot \sum_\ell \min\{m_\ell, m_\text{UB}\}\\
	&=  \frac{\alpha}{\sum_\ell m_\ell}\cdot \sum_\ell \min\{m_\ell, {m^\star}/{\alpha}\}\\
	&\leq  \frac{\alpha}{\sum_\ell m_\ell}\cdot \min\left\{ \sum_\ell m_\ell, m^\star L/\alpha\right\} = \min\left\{ \alpha, \frac{m^\star L}{\sum_\ell m_\ell}\right\}.
\end{align*}
In the above, the equality $\frac{\Delta_f}{\tilde{\Delta}_{f_\text{arr}}} = \alpha$ holds only if $m_\text{UB}\geq m_\ell$, for all $\ell \in [L]$, or equivalently, $m_\text{UB} = m^\star$. Note that in this case $\alpha = \frac{\Delta_f}{\tilde{\Delta}_{f_\text{arr}}}$ in fact equals $1$. On the other hand, the equality  $\frac{\Delta_f}{\tilde{\Delta}_{f_\text{arr}}} =\frac{m^\star L}{\sum_\ell m_\ell}\geq 1$ holds only if $m_\text{UB}\leq m_\ell$, for all $\ell\in [L]$, or equivalently, $m_\text{UB} = m_\star$. We designate $\mathsf{OPT}:= \frac{m^\star L}{\sum_\ell m_\ell}$, and note that $\Delta_f = \mathsf{OPT} \, \tilde{\Delta}_{f_\text{arr}}$ when $m_\text{UB} = m_\star$.

While the choice $m_\text{UB} = m_\star$ results in a high gain, it could potentially cause poor accuracy in estimation of the true value $f(\mathcal{D})$, due to the clipping error incurred by dropping a relatively large number of user samples. More precisely, since each array contains only very few samples,  $f_\text{arr, best}(\mathcal{D})$ could be quite different from $f(\mathcal{D})$. The next lemma shows that choosing the more favourable $m_\text{UB} = \text{med} (m_1,\ldots,m_L)$ results in a gain that is only at most a factor of 2 lower than $\mathsf{OPT}$.

\begin{lemma}
	The choice $m_\text{UB} = \text{med} (m_1,\ldots,m_L)$ results in
	\[
	\frac{\Delta_f}{\tilde{\Delta}_{f_\text{arr}}} \geq \frac{\mathsf{OPT}}{2}.
	\]
\end{lemma}
\begin{proof}
	For this choice of $m_\text{UB}$, we have that, setting $\alpha = \frac{m^\star}{m_\text{UB}}$ and $B:= \{\ell\in [L]: m_\ell< m_\text{UB}\}$,
	\begin{align*}
		\frac{\Delta_f}{\tilde{\Delta}_{f_\text{arr}}}&= \frac{\alpha}{\sum_\ell m_\ell}\cdot \sum_\ell \min\{m_\ell, m_\text{UB}\}\\
		&= \frac{\alpha}{\sum_\ell m_\ell}\cdot \left[\sum_{\ell\in B} m_\ell + \frac{m^\star\left\lceil L/2\right\rceil}{\alpha} \right]\\
		&\geq \frac{\mathsf{OPT}}{2},
	\end{align*}
since $m_\ell\geq 0$, for all $\ell\in [L]$.
\end{proof}
In our experiments in Section \ref{sec:results}, we employ $m_\text{UB} = \text{med} (m_1,\ldots,m_L)$ in demonstrating the empirical performance of \textsc{Array-Averaging} under the \textsc{BestFit} grouping strategy.
\subsection{\textsc{Levy}}
In this algorithm and the next, we attempt to reduce $\Delta_f$ further by simultaneously clipping the number of samples per user and the range of speed values. The algorithm that we present in this section puts together the \textsc{Array-Averaging} algorithm presented in the previous subsection and Algorithm 1 in \cite{userlevel}. However, unlike in the previous section, we make use of a value of $m_\text{UB}$ that is different from $\text{med} (m_1,\ldots,m_L)$ and is instead tailored, via heuristic calculations, to the sensitivity of the function associated with this algorithm.

We now present a qualitative description of the algorithm; the exact choice of the parameters is based on certain heuristics that will be described later.

As in the previous section, we first clip the number of samples contributed by any user using (one of) the array-based grouping strategies and treat the thus-formed arrays as pseudo-users. More precisely, let $A_1,\ldots,A_{\overline{K}}$ be the arrays obtained using the \textsc{BestFit} grouping strategy with a certain value of $m_\text{UB}$ to be specified later (recall that we use \textsc{BestFit} instead of \textsc{WrapAround} since under the \textsc{BestFit} strategy, a user can influence at most one array, unlike in the \textsc{WrapAround} strategy). Next, we clip the range of speed values. Suppose that $a, b$ with $0\leq a\leq b\leq U$ are real numbers such that the speed values of the users lie in $[a,b]$ with high probability. The \textsc{Levy} algorithm first privately estimates this interval $[a,b]$, with privacy loss set to $\varepsilon/2$. We then define the function
\[
f_\text{Levy}(\mathcal{D}):= \frac{1}{\overline{K}}\cdot \sum_{i=1}^{\overline{K}} \Pi_{[a,b]} (\overline{A_i}),
\]
where $\Pi_{[a,b]}$ denotes the projection operator into the interval $[a,b]$, with
\[
\Pi_{[a,b]}(x) = \min \{b, \max\{a,x\}\},
\]
for any $x\in \mathbb{R}$. As before, $\overline{A_i}:= \frac{1}{w(A_i)} \sum_{j=1}^{w(A_i)} A_i(j)$ is the mean of the samples contributed by array $i\in [\overline{K}]$. Note that now the user-level sensitivity is given by
\begin{equation}
\Delta_{f_\text{Levy}} = \frac{b-a}{\overline{K}},
\label{eq:sensitivitylevy}
\end{equation}
since we implicitly assume that grouping is performed according to the \textsc{BestFit} strategy.

The \textsc{Levy} algorithm (with \textsc{BestFit} grouping) then computes
\[
M_\text{Levy}(\mathcal{D}) = f_\text{Levy}(\mathcal{D})+\text{Lap}(2\Delta_{f_\text{Levy}}/\varepsilon).
\]
Note that in the above expression, the privacy loss is assumed to be $\varepsilon/2$. Overall, the privacy loss for both private interval estimation and for private mean estimation is $\varepsilon$, following the basic composition theorem (\cite[Corollary 3.15]{dworkroth}). Hence, the algorithm \textsc{Levy} is $\varepsilon$-DP.

Observe that when $b-a<U/2$, the standard deviation of the noise added in this case is less than that added using \textsc{Array-Averaging} with \textsc{BestFit} grouping.

We now explain the heuristics we employ to select the parameters $a, b$ in the \textsc{Levy} algorithm and $m_\text{UB}$.

\subsubsection{Private Interval Estimation}
The subroutine we use in this algorithm to privately compute the ``high-probability'' interval $[a,b]$ is borrowed from Algorithm 6 in \cite{userlevel}, which is used to privately compute an estimate of the $\left(\frac14,\frac34\right)$-interquantile interval of a given collection of i.i.d. (random) scalar values $X_1,\ldots,X_n$ (in our setting, these are the array means $\overline{A}_1,\ldots,\overline{A}_{\overline{K}}$). In order to describe this subroutine, which incorporates some additional modifications to suit our setting, we provide necessary background. The application of Algorithm 6 in \cite{userlevel} crucially relies on the following concentration property of the values $X_1,\ldots,X_n$ provided to the algorithm:
\begin{definition}
	A random sequence $X^n$ supported on $[0,M]$ is $(\tau, \gamma)$-concentrated ($\tau$ is called the ``concentration radius”) if there exists $x_0\in [0,M]$ such that with probability at least $1 - \gamma$, 
	\[
	\max_{i\in [n]} |X_i-x_0|\leq \tau.
	\]
\end{definition}

First, observe that each  ``array mean'' $\overline{A}_i$, $i\in [\overline{K}]$ is the sample mean of values $A_i(j)\in [0:U]$, where $1\leq j\leq w(A_i)$. {Although the samples in each array are drawn in a potentially non-i.i.d. fashion from an unknown distribution, we simply rely on heuristics that assume that the data samples are i.i.d. and that each array is fully filled, with $\overline{K} = K$.}

%{\color{blue} Under \textsc{BestFit} grouping, the worst case or largest sensitivity $\Delta_{f_\text{Levy}}$ corresponds to the situation where $\overline{K} = K$ (recall that $\overline{K}\geq K$, in general); in other words, the worst case senstivity corresponds to the case when $w(A_i) = m_\text{UB}$, for all $i\in [\overline{K}]$.} {\color{red} \ Anshoo: Should we rephrase the blue portion?}  

By an application of Hoeffding's inequality (see, e.g.,  \cite[Theorem 2.2.6]{vershynin}), we have that each array mean $\overline{A}_i$, $i\in [\overline{K}]$, is $\frac{U^2}{4m_\text{UB}}$-subGaussian (see, e.g., \cite[Theorem 2.1.1]{ed}). Hence, if the speed samples were i.i.d., from a simple application of the union bound (see, e.g., \cite[Theorem 2.2.1]{ed}), we obtain that the sequence $(\overline{A}_1,\ldots,\overline{A}_{\overline{K}})$ is in fact $(\tau,\gamma)$-concentrated about the expected value, where
\begin{equation}
\tau = U\cdot \sqrt{\frac{\log (2\overline{K}/\gamma)}{2m_\text{UB}}}.
\label{eq:tau}
\end{equation}
We use this value of $\tau$ to compute the ``high-probability'' interval $[a,b]$, with privacy loss $\varepsilon/2$, as shown in Algorithm \ref{alg:interval}.
\begin{algorithm}
	\caption{Private Interval Estimation}
	\begin{algorithmic}[1]
		\Procedure{PrivateInterval}{$(\overline{A}_1,\ldots,\overline{A}_{\overline{K}}), \varepsilon,\tau,U$}
		\State Divide $(0,U]$ into $U/\tau$ disjoint bins, each of width $\tau$. Let $T$ be the midpoints of the bins.
		\State Set $\mu_i\gets \min_{x\in T} |\overline{A}_i-x|$, for all $i\in [\overline{K}]$.
		\State For $x\in T$, define the cost function
		\[
		c(x) = \max \{|\{i\in [\overline{K}]: \mu_i<x\}|, |\{i\in [\overline{K}]: \mu_i>x\}|\}.
		\]
		\State Sample $\hat{\mu}\in T$ from $Q$ where
		\[
		Q(\hat{\mu}=x) = \frac{e^{-\varepsilon c(x)/4}}{\sum_{x'\in T}e^{-\varepsilon c(x')/4}}.
		\]
		\State Set $a\gets \max\left\{0,\hat{\mu}-\frac{3\tau}{2}\right\}$, $b\gets \min \left\{\hat{\mu}+\frac{3\tau}{2},U\right\}$.
		\EndProcedure
	\end{algorithmic}
	\label{alg:interval}
\end{algorithm}
\subsubsection{Choosing $m_\text{UB}$}
The subroutine we use to choose the length of the arrays $m_\text{UB}$ is tailored to the sensitivity of the function $f_\text{Levy}$ in \eqref{eq:sensitivitylevy}. For a fixed $m=m_\text{UB}$, note that from Algorithm \ref{alg:interval},
\begin{align}
	\label{eq:deltalevy}
\Delta_{f_\text{Levy}}(m)
&= \min\left\{\frac{3\tau}{\overline{K}}, \frac{U}{\overline{K}}\right\} \notag\\ &= \min\left\{\frac{3U}{\overline{K}}\sqrt{\frac{\log (2\overline{K}/\gamma)}{2m}}, \frac{U}{\overline{K}}\right\}.
\end{align}
%Under the \textsc{BestFit} grouping strategy, {\color{blue} in the worst case}, we will have that $\overline{K} = K = \left \lfloor \frac{\sum_{\ell=1}^{L}\min \left \{m_{\ell}, m \right \}}{m} \right \rfloor$ (see \eqref{eq:K}). 
In order to reduce the sensitivity, our heuristic aims to maximize the $\overline{K} \sqrt{m}$ term  in \eqref{eq:deltalevy}, and sets
\begin{equation}
	\label{eq:uboptim}
m_\text{UB} = \text{argmax}_{m} \frac{\sum_{\ell=1}^{L}\min \left \{m_{\ell}, m \right \}}{\sqrt{m}},
\end{equation}
and numerically solves this optimization problem over $m_\star\leq m\leq m^\star$.

\subsection{\textsc{Quantile}}
\label{sec:quantile}
The \textsc{Quantile} algorithm is a ``noisy mean-of-projections" that is quite similar in flavour to the \textsc{Levy} algorithm, with the only difference being the choice of the interval $[a',b']$ into which the array means are projected.

{ More precisely, the \textsc{Quantile} algorithm sets $m_\text{UB}$ as in \eqref{eq:uboptim}, and uses the \textsc{BestFit} grouping strategy to create arrays containing the speed samples.} Next, the algorithm privately estimates a ``high-probability'' interval $[a',b']$ (in a manner different from Algorithm \ref{alg:interval}), with privacy loss $\varepsilon/2$. We then define the function
\[
f_\text{Quantile}(\mathcal{D}):= \frac{1}{\overline{K}}\cdot \sum_{i=1}^{\overline{K}} \Pi_{[a',b']} (\overline{A_i}),
\]
where the projection operator and the array means are as defined earlier. Once again, we have that the sensitivity
\[
\Delta_{f_\text{Quantile}} = \frac{b'-a'}{\overline{K}},
\]
The \textsc{Quantile} algorithm (with \textsc{BestFit} grouping) then computes
\[
M_\text{Quantile}(\mathcal{D}) = f_\text{Quantile}(\mathcal{D})+\text{Lap}(2\Delta_{f_\text{Quantile}}/\varepsilon),
\]
where the privacy loss for the mean estimation is set to $\varepsilon/2$. We now describe two subroutines that we use to privately estimate the high-probability $[a',b']$.
\subsubsection{\textsc{FixedQuantile}}
This subroutine privately estimates the $\left(\frac{1}{10},\frac{9}{10}\right)$-interquantile interval of the array means $\overline{A}_1,\ldots,\overline{A}_{\overline{K}}$, using Algorithm 2 in \cite{smith}. A notable difference between this algorithm and Algorithm 6 in \cite{userlevel} (used in \textsc{Levy}) is that this algorithm does not quantize the interval $(0,U]$ in which the samples lie as in Step 2 of Algorithm \ref{alg:interval}.  Note that this algorithm computes estimates of $a'$ and $b'$ separately, and we set the privacy loss of each of these computations to be $\varepsilon/4$, so that the overall privacy loss for private quantile estimation is $\varepsilon/2$.
\subsubsection{\textsc{OptimizedQuantile}}
This subroutine privately estimates (with privacy loss $\varepsilon/2$) the interval $[a',b']$, which is now chosen to minimize the sum of the absolute estimation errors due to privacy and due to clipping the speed values, following the work in \cite{amin}. In particular, an argument similar to that in Section 3 in \cite{amin} advocates that in order to minimize this sum of absolute estimation errors, we need to set $b$ to be the $\left \lceil \frac{2}{\varepsilon}\right \rceil ^{\text{th}}$-largest value among $(\overline{A}_1,\ldots,\overline{A}_{\overline{K}})$, and by symmetry, we need to set $a$ to be the $\left \lfloor \frac{2}{\varepsilon}\right \rfloor ^{\text{th}}$-smallest value among $(\overline{A}_1,\ldots,\overline{A}_{\overline{K}})$. We then proceed to privately estimate the $\left(\frac{1}{\overline{K}}\cdot\left \lceil \frac{2}{\varepsilon}\right \rceil ,1-\frac{1}{\overline{K}}\cdot\left \lceil \frac{2}{\varepsilon}\right \rceil\right)$-interquantile interval using Algorithm 2 in \cite{smith}. Again, we set the privacy loss of computing $a'$ and $b'$ to be individually $\varepsilon/4$, so that the overall privacy loss for private quantile estimation is $\varepsilon/2$.

% Prajjwal: \subsection{Interval calculation}
%Once we group user samples into the $k$ arrays, we proceed to privately estimating an interval $\mathcal{I} = [\alpha, \beta]$ such that the means $\mathcal{Z} = \{Z_{1}, Z_{2}, ..., Z_{k}\}$ of the the arrays are concentrated within this interval. We then project the sample group means $Z_{i}$ to this interval to finally give out a differentially private estimate $\tilde{\mu}$ of the empirical mean $\mu$ after adding noise calibrated to the corresponding sensitivity $\beta - \alpha$. The motivation of interval calculation and mean projection is to achieve and improvement over the sensitivity of the samples provided as an input to the subsequent laplace mechanism and is discussed in \textit{Section C}. 
%
%To estimate the interval $\mathcal{I}$ we use the $PrivateQuantile$ algorithm proposed in [Smith11] to get a private estimate of the $q^{th}$ quantile $\alpha$ and the $(1-q)^{th}$ quantile $\beta$. In our algorithm, we use the value $q=0.1$ which would correspond to $\alpha$ and $\beta$ being the $10^{th}$ and $90^{th}$ quantiles. Thus, we would be exploiting the concentration phenomenon constituted by 80\% of the samples if any. Since the algorithm estimates the quantiles privately, a part of the privacy budget is expended for both the quantiles. Note that the algorithm can be modified to fit different choices of quantiles as well, be it symmetric or asymmetric.

% Explain the cost function
% Explain smith algo2 in brief: picking an interval and uniform draw
% Explain that the quantiles are chosen in a symmetric fashion, but the algorithm can be extended or modified for an asymmetric setting.
% Tell that the algo splits the budget to estimate the two quantiles

%Prajjwal: \begin{algorithm}
%	\caption{The private interval estimation algorithm}
%	\begin{algorithmic}[1]
%		
%		
%		\Procedure{PrivateQuantile}{$\mathcal{Z}, q, \varepsilon, a, b, \Delta$}
%		\State $Sort(\mathcal{Z})$
%		\State $k \gets \left | \mathcal{Z} \right |$
%		\State $Z_{0} \gets a, Z_{k+1} \gets b$
%		\State $y_{i} := (Z_{i+1} - Z_{i})exp(\frac{-\varepsilon \left | i - \alpha k \right |}{2\Delta})  \hspace{0.5cm} \forall i = 0, ..., k$
%		\State Sample j $\sim y_{i} / \sum_{i=0}^{k}y_{i}$
%		\State \Return $x \sim \mathcal{U}(Z_{j}, Z_{j+1})$
%		\EndProcedure
%		
%		\Procedure{PrivateInterval}{$\mathcal{S}, q, \varepsilon, a, b, \Delta$}
%		\\
%		\textit{\% The value of q should be $<$ 0.5 \%}\\
%		\textit{\% $\Delta$ is the number of arrays in $\mathcal{S}$ that can be affected by one user \%}
%		% \Comment{The value of q should be $<$ 0.5}\\
%		% \Comment{$\Delta$ is the number of arrays in $\mathcal{S}$ that can be affected by one user}
%		\State $Z_{i} := \frac{sum(S_{i})}{S_{i}.length} \hspace{0.5cm} \forall i = 1, ..., k$
%		\State $\alpha \gets PrivateQuantile(\mathcal{Z}, q, \frac{\varepsilon}{2})$
%		\State $\beta \gets PrivateQuantile(\mathcal{Z}, 1-q, \frac{\varepsilon}{2})$
%		\State \Return $\mathcal{I} = [\alpha, \beta]$
%		\EndProcedure
%	\end{algorithmic}
%\end{algorithm}

%Prajjwal: \subsection{Projection and estimation}
%The final part of the algorithm involves projecting the sample group means $Z_{i}$ to the private interval $\mathcal{I}$ followed by mean estimation and noise addition. We first estimate the mean ($\hat{\mu}$) of projected $Z_{i}$ using:
%
%\begin{equation}
%	\hat{\mu} = \frac{\sum_{i=0}^{k}\prod_{\mathcal{I}}(Z_{i})}{k}
%\end{equation}
%
%where $\prod_{\mathcal{I}}(\cdot)$ is the projection operator on interval $\mathcal{I}$.
%
%Now we make $\hat{\mu}$ private by adding noise according to the laplacian mechanism. Due to projection, the maximum change in $\sum_{i=0}^{k}\prod_{\mathcal{I}}(Z_{i})$ that can be induced by any user is restricted to $\Delta(\beta - \alpha)$ where $\Delta$ is the number of $Z_{i}$ any user can affect. This leads to the sensitivity of the corresponding mean query to be $\frac{\Delta(\beta - \alpha)}{k}.$ So it suffices for us to add noise from a Laplacian distribution with mean 0 and scale $\frac{\Delta(\beta - \alpha)}{\varepsilon k}.$ But note that we also use our privacy budget in the private estimation of the interval $\mathcal{I}.$ Hence, in order to have an overall privacy guarantee of $\varepsilon$-DP, we use expend $\varepsilon / 2$ budget in the private interval calculation and $\varepsilon / 2$ in the subsequent noise addition. Thus, our final private estimate ($\tilde{\mu}$) of the empirical mean is given by:
%
%\begin{equation}
%	\tilde{\mu} = \frac{\sum_{i=0}^{k}\prod_{\mathcal{I}}(Z_{i})}{k} + Lap(\frac{2\Delta(\beta - \alpha)}{\varepsilon k})
%\end{equation}
%
%Now we highlight the advantage of using \textsc{BestFitGrouping} algorithm over \textsc{WrapAroundGrouping}. Note that in \textsc{WrapAroundGrouping} the samples of one user can affect at most 2 arrays as the algorithm allows the samples by a user to be filled in the next array ("wrap-around") if the current array gets filled. This corresponds to $\Delta=2$. Whereas in the case of \textsc{BestFitGrouping}, the samples by one user are filled in at-most one array which gives us $\Delta=1$.

%Prajjwal: \begin{algorithm}
%	\caption{The complete algorithm using wrap-around grouping.}
%	\begin{algorithmic}[1]
%		\Procedure{PrivateMean}{$(x_i, u_i)_{i=1}^{n}, a, b, q, \varepsilon$}
%		\State $\mathcal{S} = \textsc{WrapAroundGrouping}((x_i, u_i)_{i=1}^{n})$
%		\State $\mathcal{I} = \textsc{PrivateInterval}(\mathcal{S}, q, \varepsilon / 2, a, b, 2)$
%		\State $Z_{i} := \frac{sum(S_{i})}{S_{i}.length} \hspace{0.5cm} \forall i = 1, ..., k$
%		\State $\hat{\mu} \gets \frac{\sum_{i=0}^{k}\prod_{\mathcal{I}}(Z_{i})}{k}$
%		\State $\tilde{\mu} \gets \hat{\mu} + Lap(\frac{4(\beta - \alpha)}{\varepsilon k})$
%		\State \Return $\tilde{\mu}$
%		\EndProcedure
%	\end{algorithmic}
%\end{algorithm}
%
%\begin{algorithm}
%	\caption{The complete algorithm using best-fit grouping.}
%	\begin{algorithmic}[1]
%		\Procedure{PrivateMean}{$(x_i, u_i)_{i=1}^{n}, a, b, q, \varepsilon$}
%		\State $\mathcal{S} = \textsc{BestFitGrouping}((x_i, u_i)_{i=1}^{n})$
%		\State $\mathcal{I} = \textsc{PrivateInterval}(\mathcal{S}, q, \varepsilon / 2, a, b, 1)$
%		\State $Z_{i} := \frac{sum(S_{i})}{S_{i}.length} \hspace{0.5cm} \forall i = 1, ..., k$
%		\State $\hat{\mu} \gets \frac{\sum_{i=0}^{k}\prod_{\mathcal{I}}(Z_{i})}{k}$
%		\State $\tilde{\mu} \gets \hat{\mu} + Lap(\frac{2(\beta - \alpha)}{\varepsilon k})$
%		\State \Return $\tilde{\mu}$
%		\EndProcedure
%	\end{algorithmic}
%\end{algorithm}


==> results.tex <==
\label{sec:results}
\subsection{Setup}

\begin{figure*}[]
	\centering
	\includegraphics[width=\linewidth]{grouping2.png}
	\caption{Plots comparing $E_\text{MAE}$ for the \textsc{Array-Averaging}, \textsc{Levy}, and \textsc{Quantile} algorithms, under the two grouping strategies. For the \textsc{Levy} algorithm, we fix $\gamma = 0.2$, and for the \textsc{Quantile} algorithm, we use the \textsc{FixedQuantile} subroutine.}
	\label{fig:group}
\end{figure*}

%Prajjwal: We compare our algorithms with two approaches. The first approach is a baseline which involves the naive use of laplace mechanism in which laplace noise is added with sensitivity $\frac{(b-a)m^{*}}{\sum_{i=1}^{n}m_{i}}$ where $m^{*}$ is the maximum number of samples contributed by any user. Thus the final estimate $\mu_{base1}$ is given by :
%
%\begin{equation}
%	\mu_{base1} = \frac{\sum_{i=1}^{n} \sum_{j=1}^{m_{i}} x_{j}}{\sum_{k=1}^{n} m_{k}} + Lap(\frac{(b-a)m^{*}}{\sum_{p=1}^{n}m_{p}\varepsilon})
%\end{equation}
%
%The second approach is the algorithm proposed by Levy et. al in [Lev+21]. Their algorithm considers the case in which all users contribute same number of samples. So in order to fit their approach to out setting, we modify and extend their algorithm with \textsc{WrapAroundGrouping}. Note that their approach assumes samples drawn i.i.d from a sub-Gaussian distribution, and hence is not expected to give optimal results in a non-i.i.d setting. Additionally \textsc{BestFitGrouping} cannot be used in conjunction with their approach as the subsequent "Median of Means" algorithm for interval calculation requires all samples groups to be completely filled in order to exploit the concentration property contained by the coarse mean $\mu_{c}$ and $\tau$. $\tau$ is a constant which is given by $\sigma \sqrt{ \frac{2}{l} log(\frac{2k}{\gamma} ) }$. The interval estimated by [Lev+21] is given by $\mathcal{I}_{Levy}$[$\bar{\mu} - 1.5\tau$, $\bar{\mu} + 1.5\tau$] where $\bar{\mu}$ is the private median of means. Thus, the sensitivity of the mean of $Z_{i}$ after projecting them to this interval is limited to $\frac{3\tau}{k}$. Thus the final estimate using Levy et al.'s approach is given by:
%
%\begin{equation}
%	\mu_{levy} = \frac{\sum_{i=0}^{k}\prod_{\mathcal{I}_{levy}}Z_{i}}{k} + Lap(\frac{12\tau}{k\varepsilon})
%\end{equation}
%
%For comparing our algorithm with their approach,  we set $\gamma = 0.2$ which corresponds to the probability that any mean $Z_{i}$ would lie beyond the interval returned by the algorithm. Since in our algorithm, $\alpha$ and $\beta$ correspond to the $10^{th}$ and $90^{th}$ quantiles respectively, we are effectively winsorizing 20\% of $Z_{i}$ which makes the comparison fair with [Lev+21] with $\gamma = 0.2$.


{We test and evaluate our algorithms on two types of datasets: 1) a real-world ITMS dataset containing non-i.i.d. speed values contributed by bus drivers over a span of 3 days in an Indian city, and 2) a synthetic dataset containing i.i.d. samples drawn using insights from the ITMS data. We ran each private mean estimation algorithm described in Section \ref{sec:alg} $10^4$ times; the plots showing the performance of our algorithms are shown in this section. We test the accuracy of our algorithms, via the error in estimation, for privacy loss $\varepsilon$ ranging from $0.5$ to $2$.}

We use the mean absolute error (or MAE) metric, $$E_\text{MAE}(\mathcal{C}) = {\frac{\sum_{i=0}^{10^4} \left \lvert M^{(i)}(\mathcal{C}) - \mu(\mathcal{C})\right \lvert}{10^4}}$$ to evaluate the performance of the algorithm. Here, for $i\in [10^4]$, $M^{(i)}(\mathcal{C})$ is the result of running the algorithm $M$ (which is one of  \textsc{Array-Averaging}, \textsc{Levy}, and \textsc{Quantile}, with a choice of subroutines) on the dataset $\mathcal{C}$ at iteration $i$, and $\mu(\mathcal{C})$ is the true sample mean.  Since, for $Z\sim \text{Lap}(b)$, we have $\E[|Z|] = b$, we simply use $E_\text{MAE}(\mathcal{C}) = \Delta_f/\varepsilon$ for \textsc{Baseline}.

% How to write the percentile formula ?

\subsection{Experimental Results for ITMS Data}



For our ITMS dataset $\mathcal{D}$, the number of users $L=217$, the maximum and minimium number of samples contributed by any user are respectively $m^{*} = 417$ and $m_* = 1$, and the total number of samples contributed by all user was $\sum_\ell m_\ell = 17166$. The true sample mean of speed records $\mu(\mathcal{D})$ was $20.66769$. We also mention that we pick $\text{med}(m_1,\ldots,m_L) = 46$. {Also, for  $m_\text{UB}$ as in \eqref{eq:uboptim}, the number of arrays $K$ under \textsc{WrapAround} grouping was $160$ and the number of arrays $\overline{K}$ under  \textsc{BestFit} grouping was $164$.}
%{\color{red} \ Anshoo: $m_\text{UB}$ computed using \eqref{eq:uboptim}? (see spcom version).} 

%Prajjwal: Thus for the naive approach we are adding laplace noise with scale 1.5789/$\varepsilon$. The calculated value of $\tau$ for [Lev+21] algorithm came out to be 18.4069. Thus, this approach would involve addition of laplace noise with scale $1.380/\varepsilon$. Note that in our and [Levy+21]'s algorithms, the resulting error is not only because of the noise term but also due to coarse estimate of mean (mean of projected values) as well.

First, we compare the performance of the algorithms that employ clipping of the number of user samples, under \textsc{WrapAround} and \textsc{BestFit} grouping strategies. In particular, we evaluate $E_\text{MAE}$ for \textsc{Array-Averaging}, for \textsc{Levy} with $\gamma = 0.2$, and for \textsc{Quantile}, with the \textsc{FixedQuantile} subroutine, under the two grouping strategies. Figure \ref{fig:group} shows these comparisons, for $\varepsilon$ varying from $0.5$ to $2$. While for the \textsc{Array-Averaging} algorithm, the performance of the two grouping strategies is similar, it is clear from the plots that for the \textsc{Levy} and \textsc{Quantile} algorithms, the \textsc{BestFit} strategy performs much better than the \textsc{WrapAround} strategy. This conforms with our expectation (see the discussion in Section \ref{sec:grouping}, since the \textsc{WrapAround} strategy results in a multiplicative factor of $2$ in the user-level sensitivity).

In Figure \ref{fig:itmscompare}, we hence fix the grouping strategy to be \textsc{BestFit} and compare the performance of the 4 algorithms described in Section \ref{sec:alg} on the non-i.i.d. ITMS dataset. Clearly, clipping of the number of samples per user and the speed values results in much better performance than the na\"{i}ve \textsc{Baseline} approach. However, there is very little difference between the performance of the other algorithms, possibly owing to the relatively small size of the ITMS dataset.

%Prajjwal: [Levy+21]'s approach results in 1.369 $l_{2}$ error for $\varepsilon=1.8$ whereas a similar error of 1.3854 is obtained using our algorithm with \textsc{BestFitGrouping} with $\varepsilon=0.6$, resulting a 3 times improvement over the privacy budget.

%\begin{figure}[!t]
%	\centering
%	\includegraphics[width=\linewidth]{GroupingAlgoComparisonArrayAveraging_NS.png}
%	\caption{Plots comparing $E_\text{RMSE}$ and $E_\text{MAE}$ for the \textsc{Array-Averaging} algorithm under the two grouping strategies.}
%	\label{fig:group1}
%\end{figure}
%
%\begin{figure}[]
%	\centering
%	\includegraphics[width=\linewidth]{GroupingAlgoComparisonLevy_NS.png}
%	\caption{Plots comparing $E_\text{RMSE}$ and $E_\text{MAE}$ for the \textsc{Levy} algorithm, with $\gamma = 0.2$, under the two grouping strategies.}
%	\label{fig:group2}
%\end{figure}
%
%\begin{figure}[!h]
%	\centering
%	\includegraphics[width=\linewidth]{GroupingAlgoComparisonQuantile_NS.png}
%	\caption{Plots comparing $E_\text{RMSE}$ and $E_\text{MAE}$ for the \textsc{Levy} algorithm, with $\gamma = 0.2$, under the two grouping strategies.}
%	\label{fig:group3}
%\end{figure}



% Do we need this? \begin{figure}[!h]
%	\centering
%	\includegraphics[width=3.4in]{rmse.png}
%	
%	\caption{$l_{2}$ error vs Epsilon graph}
%	\label{rmse}
%\end{figure}
%
%
%Do we need this? \begin{figure}[!h]
%	\centering
%	\includegraphics[width=3.4in]{perc.png}
%	\caption{95th percentile error vs Epsilon graph}
%	\label{perc95}
%\end{figure}

\subsection{Experimental Results for Synthetic Data}

Next, we artificially generate data samples, by drawing insights from the ITMS dataset. This artificially generated dataset, denoted as $\mathcal{D}'$, allows us to study the performance of the algorithms in Section \ref{sec:alg} when the number of samples per user or the number of users is large. In particular, let $\widehat{L}$ denote the number of users and $\widehat{m_\ell}$, for $\ell \in [\widehat{L}]$ denote the number of samples contributed by user $\ell$. Recall that $L$ and $\{m_\ell: \ell \in [L]\}$ denoted the number of users and the collection of the number of samples per user for the original ITMS dataset. We generate i.i.d. speed samples $\left\{\widehat{S}_j^{(\ell)}: \ell \in [\widehat{L}], j\in [\widehat{m_\ell}]\right\}$, where for any $\ell, j$, we have $\widehat{S}_j^{(\ell)}\sim \Pi_{[0,U]}(X)$, where $X\sim \mathcal{N}(\mu(\mathcal{D}),\sigma^2(\mathcal{D}))$. Here, $\mu(\mathcal{D})$ is the true sample mean of the ITMS dataset and $\sigma^2(\mathcal{D})$ is the true sample variance of the ITMS dataset, defined as
\[
\sigma^2(\mathcal{D}) = \frac{1}{\sum_{\ell=1}^{L}{m_\ell}}\cdot \sum_{\ell=1}^L \sum_{j=1}^{m_\ell}\left(S_j^{(\ell)}-\mu(\mathcal{D})\right)^2.
\]
For the ITMS dataset, $\sigma^2(\mathcal{D}) = 115.135$. Further, note that the  random variable $\widehat{S}_j^{(\ell)}$ obeys:
\begin{align*}
\Pr\left[\widehat{S}_j^{(\ell)} = 0\right] &= Q\left(\frac{\mu(\mathcal{D})}{\sigma(\mathcal{D})}\right)\ \text{and}\\ \Pr\left[\widehat{S}_j^{(\ell)} = U\right] &= Q\left(\frac{U-\mu(\mathcal{D})}{\sigma(\mathcal{D})}\right).
\end{align*}
  In what follows, we set $\mu := \mu(\mathcal{D})$ and $\sigma^2 := \sigma^2(\mathcal{D})$. We consider two settings of interest, for a fixed positive integer $\lambda$.
\begin{enumerate}
	\item \textbf{Sample scaling}: In this setting, we set $\widehat{L} = L$ and $\widehat{m}_\ell = 10\cdot m_\ell$, for all $\ell\in [\widehat{L}]$. In this case, $\widehat{m}^\star := \max_{\ell\in [\widehat{L}]} \widehat{m}_\ell = \lambda\cdot m^\star$. 
	\item \textbf{User scaling}: In this setting, we set $\widehat{L} = \lambda\cdot L$ where $\lambda$ is a positive integer. For each $i\in [\lambda]$, we let $\widehat{m}_{\lambda\cdot(\ell-1)+i} = m_\ell$,  for all $\ell\in [{L}]$. Here, $\widehat{m}^\star = m^\star$.
\end{enumerate}

We also let $\widehat{m}_\text{UB}$ denote the new lengths of the arrays used for the dataset $\mathcal{D}'$, with $\widehat{K}$ and $\widehat{\overline{K}}$ denoting, respectively, the resultant number of arrays under the \textsc{WrapAround} and \textsc{BestFit} grouping strategies. Further, for each of the algorithms considered in Section \ref{sec:alg}, we denote their sensitivities under sample scaling (resp. user scaling) by using an additional superscript `$(s)$' (resp. `$(u)$') over the existing notation.

We first consider the setting of \textbf{sample scaling}, with $\lambda = 10$. Figure \ref{fig:samplescale} shows comparisons between the different algorithms on this synthetic dataset, with $\gamma = 0.2$ for \textsc{Levy}. Here, we implicitly assume that the grouping strategy employed is \textsc{BestFit}. It is evident from the plots that \textsc{Baseline} performs much poorer than the clipping algorithms, as expected. However, interestingly, the \textsc{Levy} algorithm performs better than all other algorithms. 
%To understand why, we first introduce some notation: let $\Delta^{(s)}_{f_\text{Baseline}}, \Delta_{f_\text{arr, wrap}}^{(s)}, \Delta_{f_\text{arr, best}}^{(s)}, \Delta_{f_\text{Levy}}^{(s)},$ $ \Delta_{f_\text{FixedQuantile}}^{(s)}$, and  $\Delta_{f_\text{$\varepsilon$-DepQuantile}}^{(s)}$ denote the sensitivities for the algorithms (with specific choices of subroutines) considered in Section \ref{sec:alg}, under sample scaling.  We mention that for \textsc{Levy} and \textsc{Quantile}, we use the \textsc{BestFit} grouping strategy. 

To see why, we first need the following simple lemma.

\begin{lemma}
	\label{lem:samplescale}
	Under sample scaling, we have that 
	\[
	\widehat{m}_\text{UB} = \lambda\cdot m_\text{UB},\ \widehat{K} = K,\ \text{and}\ \widehat{\overline{K}} = \overline{K},
	\]
	for $m_\text{UB}$ chosen either as the sample median or as in \eqref{eq:uboptim}.
\end{lemma}
We now proceed to justify the performance trends observed under sample scaling, by analyzing the dependence of the sensitivities on the scaling factor.

\begin{proposition}
	We have that
	\begin{align*}
	\Delta^{(s)}_{f_\text{Baseline}} = \Delta_{f_\text{Baseline}},\
	\Delta^{(s)}_{f_\text{arr, wrap}} = \Delta_{f_\text{arr, wrap}},\ \Delta^{(s)}_{f_\text{arr, best}} = \Delta_{f_\text{arr, best}},
	\end{align*}
and 
\[
\Delta^{(s)}_{f_\text{Levy}} = \frac{1}{\sqrt{\lambda}}\cdot  \Delta_{f_\text{Levy}}.
\]
\end{proposition}
\begin{proof}
	The above scaling of the sensitivities under sample scaling follows directly from the definitions of the sensitivities and from Lemma \ref{lem:samplescale}.
\end{proof}

%The justification for this superior performance of \textsc{Levy} in the sample scaling setting is as follows. First, observe that in the \textsc{Levy} algorithm, from the optimization problem \eqref{eq:uboptim} that computes the length of the arrays, we now have that the length of the arrays
%\[
%\widehat{m}_\text{UB} = \text{argmax}_{m} \frac{\sum_{\ell=1}^{L}\min \left  \{10\cdot m_{\ell}, m \right \}}{\sqrt{m}}.
%\]
%Clearly, the choice $\widehat{m}_\text{UB} = 10\cdot m_\text{UB}$ solves this optimization problem, where $m_\text{UB}$ was the length of the arrays used in the absence of sample scaling. Furthermore, with this choice of the length of arrays used, the number of arrays $\widehat{\overline{K}}$ obtained using \textsc{BestFit} grouping equals $\overline{K}$. Hence, we have that the user-level sensitivity using the \textsc{Levy} algorithm (see \eqref{eq:deltalevy}) is
%\[
%\Delta_{f_\text{Levy}}(\widehat{m}_\text{UB}) = \frac{3U}{\overline{K}}\sqrt{\frac{\log (2\overline{K}/\gamma)}{20m_\text{UB}}},
%\]
%which is a factor $1/\sqrt{10}$ smaller than the user-level sensitivity without scaling. In general, when the number of samples per user is scaled by a factor of $\lambda>1$, we get a multiplicative factor of $1/\sqrt{\lambda}$ improvement in the user-level sensitivity, and hence in the standard deviation of the noise added, thereby improving performance. {
%In contrast, the sensitivity for \textsc{Baseline} (see \eqref{eq:delf}), and the sensitivity for \textsc{Array-Averaging} (see \eqref{eq:delfbest}) remain unchanged from the corresponding values without sample scaling.} 

It is clear from the above proposition that the sensitivity (and hence the amount of Laplace noise added for privacy) is much smaller for \textsc{Levy} as compared to \textsc{Baseline} and \textsc{Array-Averaging}, for large enough $\lambda$. 

Now, for the case of the \textsc{Quantile} algorithm, a precise analysis of the sensitivity of the algorithm as stated is hard, owing to possible errors in the private estimation of the quantiles used.
%we consider the situation where we set $a'$ and $b'$ (see Section \ref{sec:quantile}) to represent the ``true'' quantiles that depend on the distribution of the samples and not on the samples themselves. More precisely, we let $a'$ and $b'$ to be such that
%\begin{equation}
%\Pr\left[\widehat{\overline{A}}_1<a'\right] = q,\ \text{and}\ \Pr\left[\widehat{\overline{A}}_1\geq b'\right] = 1-q,
%\label{eq:a_bar}
%\end{equation}
%with $q = 1/10$, under \textsc{FixedQuantile}, and $q = {\widehat{\overline{K}}}^{-1}\cdot\left \lceil \frac{2}{\varepsilon}\right \rceil$, under \textsc{$\varepsilon$-DependentQuantile}. Here, the random variable $\widehat{\overline{A}}_1$ represents the array mean of array $\widehat{A}_1$. Further, we assume that each of the arrays used in the \textsc{Quantile} algorithm is fully filled. The following result then holds.
%\begin{proposition}
%	If the true distribution-dependent quantiles are used, we have that if $q\leq \min\{Q(\mu/\sigma),1-Q((U-\mu)/\sigma)\}$, then
%	$
%	\Delta^{(s)}_{f_\text{Quantile}} =
%		\frac{U}{\widehat{\overline{K}}}.
%	$
%%	$
%%	\Delta^{(s)}_{f_\text{Quantile}} = \frac{1}{\sqrt{\lambda}}\cdot \Delta_{f_\text{Quantile}},
%%	$
%%	under both \textsc{FixedQuantile} and \textsc{$\varepsilon$-DependentQuantile}.
%\end{proposition}
%\begin{proof}
%	First, recall that $\widehat{S}_1^{(1)}\sim \mathcal{N}(\mu,\sigma^2)$, where $\mu := \mu(\mathcal{D})$ and $\sigma^2 := \sigma^2(\mathcal{D})$. Assuming that each array is fully filled, we have that $\widehat{\overline{A}}_i\sim \mathcal{N}(\mu,\sigma^2/\widehat{m}_\text{UB})$. It is then clear that choosing 
%	$$a' = \frac{\mu\cdot \sqrt{\widehat{m}_\text{UB}}-\sigma\cdot Q^{-1}(q)}{\sqrt{\widehat{m}_\text{UB}}}\ \text{and}\ b' = \frac{\mu\cdot \sqrt{\widehat{m}_\text{UB}}+\sigma\cdot Q^{-1}(q)}{\sqrt{\widehat{m}_\text{UB}}}$$ makes \eqref{eq:a_bar} hold.
%	
%	Hence, the sensitivity $$\Delta^{(s)}_{f_\text{Quantile}} = \frac{b'-a'}{\widehat{\overline{K}}} = \frac{2\sigma\cdot Q^{-1}(q)}{\sqrt{\widehat{m}_\text{UB}}\cdot \widehat{\overline{K}}}.$$
%	
%	The proof is concluded by appealing to Lemma \ref{lem:samplescale}, which shows that $\widehat{\overline{K}}$ and $q$ remain unchanged under sample scaling, but $\widehat{m}_\text{UB} = \lambda\cdot m_\text{UB}$.
%\end{proof}
%While both the \textsc{Levy} and \textsc{Quantile} algorithms show a reduction in sensitivity by a multiplicative factor of $1/\sqrt{\lambda}$, 
We believe the relative better performance of \textsc{Levy} is due the additional errors in private estimation of the quantiles in \textsc{Quantile}. Hence, in general, when the dataset contains a large number of samples per user, we recommend using \textsc{Levy}.

Figure \ref{fig:userscale} for \textbf{user scaling} shows that the \textsc{FixedQuantile} subroutine outperforms all the other algorithms. Furthermore, \textsc{Array-Averaging} performs second-best. We mention that here we use $m_\text{UB}$ as in \eqref{eq:uboptim} for \textsc{Array-Averaging} as well, to maintain uniformity. We now justify these performance trends. Analogous to the setting with sample scaling, the following simple lemma holds.
\begin{figure}[!h]
	\centering
	\includegraphics[width=0.9\linewidth]{itms.png}
	\caption{Plots comparing the performance of algorithms on real-world ITMS data}
	\label{fig:itmscompare}
\end{figure}

%Do we need this? \begin{figure}[!h]
%	\centering
%	\includegraphics[width=3.4in]{ConcentrationAlgoComparisonBestFit_SS.png}
%	\caption{95th percentile error vs Epsilon graph}
%	\label{perc95}
%\end{figure}



%\begin{figure}[!h]
%	\centering
%	\includegraphics[width=3.4in]{ConcentrationAlgoComparisonBestFit_SynthUser+BS.png}
%	\caption{95th percentile error vs Epsilon graph}
%	\label{perc95}
%\end{figure}

\begin{figure}[!h]
	\centering
	\includegraphics[width=0.9\linewidth]{sample-scaling.png}
	\caption{Plots comparing the performance of algorithms under \textbf{sample scaling}}
	\label{fig:samplescale}
\end{figure}

\begin{figure}[!h]
	\centering
	\includegraphics[width=0.9\linewidth]{user-scaling.png}
	\caption{Plots comparing the performance of algorithms under \textbf{user scaling}}
	\label{fig:userscale}
\end{figure}
\begin{lemma}
	\label{lem:user_scale}
	Under user scaling, we have that 
	\[
	\widehat{m}_\text{UB} = m_\text{UB},\ \widehat{K} = \lambda\cdot K,\ \text{and}\ \widehat{\overline{K}} = \lambda\cdot \overline{K},
	\]
	for $m_\text{UB}$ chosen as in \eqref{eq:uboptim}.
\end{lemma}
With the above lemma in place, we first provide a justification of the superior performance of \textsc{Array-Averaging}, compared to \textsc{Levy} and \textsc{$\varepsilon$-DependentQuantile}, where we assume that the exact sample-dependent quantiles are computed in \textsc{$\varepsilon$-DependentQuantile} (i.e., we assume that the error in estimation of the sample quantiles due to privacy is zero). To  denote the standard deviation of noise added in each algorithm described in Section \ref{sec:alg}, under user scaling, we use the same notation as for the sensitivities under user scaling, but replacing $\Delta$ with $\sigma$. We recall that for $X \sim \mathrm{Lap}(b)$, the standard deviation of $X$, denoted by $\sigma$, is $\sqrt{2} b$. We implicitly assume that \textsc{BestFit} is used as the grouping strategy in each algorithm.
\begin{proposition}
 For any fixed $\varepsilon$, for large enough $\lambda$, we have that with high probability, $$\sigma^{(u)}_{f_\text{arr, best}}< \min\left\{ \sigma^{(u)}_{f_\text{Levy}}, \sigma^{(u)}_{f_\text{Quantile}}\right\},$$ under the \textsc{$\varepsilon$-DependentQuantile} subroutine for \textsc{Quantile}, if the exact sample quantiles are employed.
\end{proposition}

\begin{proof}
	First consider \textsc{Array-Averaging} under user scaling. Recall that $\Delta^{(u)}_{f_\text{arr, best}} = \frac{U}{\widehat{\overline{K}}} = \frac{U}{\lambda\cdot {\overline{K}}}$, where the last equality follows from Lemma \ref{lem:user_scale}. Hence, we have that $\sigma^{(u)}_{f_\text{arr, best}} = \frac{\sqrt{2}U}{\lambda{\overline{K}}\varepsilon}$.
	
	Now, consider \textsc{Levy} under user scaling. From \eqref{eq:deltalevy}, we have that 
	\[
	\sigma_{f_\text{Levy}}^{(u)}
	= \min\left\{\frac{6\sqrt{2}\cdot\tau}{\widehat{\overline{K}}\cdot \varepsilon}, \frac{2\sqrt{2}\cdot U}{\widehat{\overline{K}}\cdot \varepsilon}\right\} = \frac{2\sqrt{2}\cdot U}{\lambda{\overline{K}}\varepsilon},
	\]
	for $\lambda\geq \frac{\gamma}{2\overline{K}}\cdot e^{2m_\text{UB}/9}$ (see \eqref{eq:tau}). Here, in the last equality above, we once again invoke Lemma \ref{lem:user_scale} to obtain $$\widehat{\tau} =  U\cdot \sqrt{\frac{\log (2\lambda\overline{K}/\gamma)}{2m_\text{UB}}}.$$ Hence, for $\lambda\geq \frac{\gamma}{2\overline{K}}\cdot e^{2m_\text{UB}/9}$, we have that $\sigma^{(u)}_{f_\text{arr, best}}< \sigma^{(u)}_{f_\text{Levy}}$.
	
	Now consider the \textsc{$\varepsilon$-DependentQuantile} under user scaling. Fix some $\delta>0$ such that $\delta<U/4$. We claim that for large enough $\lambda$, the true $\left({\widehat{\overline{K}}}^{-1}\cdot\left \lceil \frac{2}{\varepsilon}\right \rceil ,1-{\widehat{\overline{K}}}^{-1}\cdot\left \lceil \frac{2}{\varepsilon}\right \rceil\right)$-interquantile interval of the samples contains $[\delta,U-\delta]$, with high probability. To this end, let $t := \left \lceil \frac{2}{\varepsilon}\right \rceil$ and let $B$ denote the event that $\left({\widehat{\overline{K}}}^{-1}\cdot{t},1-{\widehat{\overline{K}}}^{-1}\cdot{t}\right)$-interquantile interval is contained in $[\delta,U-\delta]$. We shall now show that $\Pr[B]$ decays to zero as $\lambda$ increases to infinity. Observe that
	\begin{align}
	&\Pr\left[B\right] \notag\\
	&\leq \Pr\left[\exists\ {\widehat{\overline{K}}}-2t \text{ array means all lying in } [\delta,U-\delta]\right]. \label{eq:inter}
	\end{align}
Now, let $B_i$ denote the event that $\widehat{\overline{A}}_i$, for $i\in [\widehat{\overline{K}}]$ lies in $[\delta,U-\delta]$, and let $i^\star$ denote that array index $i$ that maximizes $\Pr[B_i]$. Note that 
\[
\Pr[B_{i^\star}]\leq 1-\max\left\{\Pr[\widehat{\overline{A}}_{i^\star} = 0], \Pr[\widehat{\overline{A}}_{i^\star} = U]\right\}.
\]

Further, we have that
\begin{align*}
\Pr[\widehat{\overline{A}}_{i^\star} = 0] &= \left(\Pr[\widehat{S}_1^{(1)} = 0]\right)^{w(\widehat{A}_{i^\star})}\\
&= (1-Q(\mu/\sigma))^{w(\widehat{A}_{i^\star})}>0.
\end{align*}
where we use the fact that the samples $\widehat{S}_j^{(\ell)}$, $\ell\in [\widehat{L}]$, $j\in [\widehat{m}_\ell]$ are drawn i.i.d. according to the ``projected'' Gaussian distribution described earlier. Since $w(\widehat{A}_{i^\star})>0$, we get that $\Pr[\widehat{\overline{A}}_{i^\star} = 0]>0$ and hence that $\Pr[B_{i^\star}]<1$.
%Since each sample $\widehat{S}_j^{\ell}\sim \mathcal{N}(\mu, \sigma^2)$, \textcolor{red}{Arvind: This here is not correct, given the projection procedure. I think we will require an assumption that the arrays are all fully filled, since I have not been able to obtain a neat closed-form expression for the sum of ``projected'' Gaussians} independently across samples, for $\ell \in \widehat{L}$ and $j\in [\widehat{m}_\ell]$, we get that each array mean $\widehat{\overline{A}}_i$, $1\leq i\leq \widehat{\overline{K}}$ is normally distributed, with mean $\mu$ and variance $\sigma^2/w(\widehat{\overline{A}}_i)$, where $w(\widehat{\overline{A}}_i)$ is the number of filled locations in array $\widehat{\overline{A}}_i$. Let $i^\star$ denote the index of that array that is filled the most, i.e., $\widehat{\overline{A}}_{i^\star}\geq \widehat{\overline{A}}_{i}$, for all $i$. Clearly, we have that for all $i\in \widehat{\overline{K}}$,


%\[\Pr\left[\widehat{\overline{A}}_i\in [\delta,U-\delta]\right] \leq \Pr\left[\widehat{\overline{A}}_{i^\star}\in [\delta,U-\delta]\right]\in (0,1).\]
Employing a union bound argument to upper bound the probability in \eqref{eq:inter}, we get that
\begin{align*}
	\Pr[B]&\leq \binom{{\widehat{\overline{K}}}}{{\widehat{\overline{K}}}-2t}\cdot \prod_{i=1}^{\widehat{\overline{K}}}\Pr\left[B_i\right]\\
	&\leq \binom{{\widehat{\overline{K}}}}{{\widehat{\overline{K}}}-2t}\cdot \big(\Pr\left[B_{i^\star}\right]\big)^{\widehat{\overline{K}}} = \binom{{\widehat{\overline{K}}}}{2t}\cdot \big(\Pr\left[B_{i^\star}\right]\big)^{\widehat{\overline{K}}}
\end{align*}
where the second inequality holds by the definition of $i^\star$.
Since $\binom{{\widehat{\overline{K}}}}{2t}$ grows polynomially in $\lambda$, for a fixed $t$ (see Lemma \ref{lem:user_scale}), we have that for any fixed $\delta>0$, and for a fixed, small $\beta\in (0,1)$, there exists $\lambda_0$, such that for all $\lambda\geq \lambda_0$, we have that $\Pr[B]<\beta$.

%Therefore, taking $\delta\downarrow 0$, we obtain that with high probability, the $\left(\frac{t}{\widehat{\overline{K}}},1-\frac{t}{\widehat{\overline{K}}}\right)\text{-interval}$ equals $[0,U]$.

Therefore, for any arbitrarily small $\beta > 0$ and for $\lambda\geq \lambda_0$, we have that with probability at least $1-\beta$,
\[
\sigma^{(u)}_{f_\text{Quantile}}
\geq \frac{2\sqrt{2}\cdot(U-2\delta)}{\widehat{\overline{K}}\cdot \varepsilon}> \frac{\sqrt{2}\cdot U}{\widehat{\overline{K}}\cdot \varepsilon} =  \sigma^{(u)}_{f_\text{arr, best}},
\]
where the second inequality holds since $\delta< U/4$.

Hence, by picking $\lambda\geq \max\left\{\lambda_0,\frac{\gamma}{2\overline{K}}\cdot e^{2m_\text{UB}/9}\right\}$, we get $\sigma^{(u)}_{f_\text{arr, best}}< \min\left\{ \sigma^{(u)}_{f_\text{Levy}}, \sigma^{(u)}_{f_\text{Quantile}}\right\},$ with probability at least $1-\beta$.
\end{proof}

All that remains is to show that the \textsc{FixedQuantile} algorithm performs better than \textsc{Array-Averaging}. By arguments similar to those above, we observe that since the \textsc{FixedQuantile} subroutine eliminates a much larger fraction of data samples in the computation of $[a',b']$, with high probability, we have that $b'-a'$ is small, and hence the amount of noise added in this case is lower than that for \textsc{Array-Averaging}. Hence, in general, for datasets with a large number of users, we recommend using \textsc{FixedQuantile}.


